Relational Fusion Networks: Graph Convolutional Networks for Road Networks

The application of machine learning techniques in the setting of road networks holds the potential to facilitate many important intelligent transportation applications. Graph Convolutional Networks (GCNs) are neural networks that are capable of leveraging the structure of a network. However, many implicit assumptions of GCNs do not apply to road networks. We introduce the Relational Fusion Network (RFN), a novel type of GCN designed specifically for road networks. In particular, we propose methods that outperform state-of-the-art GCNs by 21%-40% on two machine learning tasks in road networks. Furthermore, we show that state-of-the-art GCNs may fail to effectively leverage road network structure and may not generalize well to other road networks.

==> frontmatter.tex <==
\title{Relational Fusion Networks:\\Graph Convolutional Networks for Road Networks}
\author{Tobias Skovgaard Jepsen, Christian S. Jensen, and Thomas Dyhre Nielsen%
\thanks{Manuscript received by ... %
  The research presented in this paper is supported in part by the DiCyPS project and by grants from the Obel Family Foundation and VILLUM FONDEN.
We also thank the \glsfirst{osm} contributors who have made this work possible.
Map data is copyrighted by the OpenStreetMap contributors and is available from {https://www.openstreetmap.org}.
All authors are affiliated with the Department of Computer Science at Aalborg University.}
}
\IEEEpubid{}

\maketitle


==> illustrations/architecture.tikz.tex <==
\usetikzlibrary{shapes,arrows,positioning}
\begin{tikzpicture}[
    align=center,
    layer/.style={shape=rectangle, text width=2cm, align=center, draw=black} 
  ]
  \def\layerdistance{0.5cm}
   % Input Layer
    \node[] (Xn) at (0,0) {$X^V$};
    \node[] (Xe) at (3,0) {$X^E$};
    \node[] (Xbe) at (6,0) {$X^{B}$};

   % Layer 1
    \node[layer, above=0.5cm of Xn] (GCN1n) {Primal Graph Convolution};
    \draw[->] (Xn) -- (GCN1n);
    \draw[->] (Xe) -- (GCN1n);
    
    \node[layer, above=0.5cm of Xe] (GCN1e) {Dual Graph Convolution};
    \draw[->] (Xn) -- (GCN1e);
    \draw[->] (Xe) -- (GCN1e);
    \draw[->] (Xbe) -- (GCN1e);

    \node[layer, above=0.5cm of Xbe] (FF1be) {Feed\\Forward};
    \draw[->] (Xbe) -- (FF1be);
    
   % Layer 2
    \node[layer, above=1cm of GCN1n] (GCN2n) {Primal Graph Convolution};
    \draw[->] (GCN1n) -- (GCN2n);
    \draw[->] (GCN1e) -- (GCN2n);
    
    \node[layer, above=1cm of GCN1e] (GCN2e) {Dual Graph Convolution};
    \draw[->] (GCN1e) -- (GCN2e);
    \draw[->] (GCN1n) -- (GCN2e);
    \draw[->] (FF1be) -- (GCN2e);
    
    \node[layer, above=1cm of FF1be] (FF2be) {Feed\\Forward};
    \draw[->] (FF1be) -- (FF2be);

    % Output Layer
    \node[layer, above=1cm of GCN2e] (GCN3e) {Dual Graph Convolution};
    \draw[->] (GCN2e) -- (GCN3e);
    \draw[->] (GCN2n) -- (GCN3e);
    \draw[->] (FF2be) -- (GCN3e);

    \node[above=0.5cm of GCN3e] (output) {Output};
    \draw[->] (GCN3e) -- (output);
\end{tikzpicture}


==> preamble.tex <==
\usepackage{verbatim}
\usepackage{placeins}
\usepackage{multirow}
\usepackage{textcomp}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumitem}
\usepackage{setspace}
\usepackage{subcaption}
\usepackage{natbib}
\usepackage{pgf}
%\usepackage[backend=bibtex,style=ieee,natbib=true]{biblatex}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\makeatletter
\renewcommand{\ALG@beginalgorithmic}{\small}
\makeatother
\algnewcommand\Input{\textbf{Input:\space}}
\algnewcommand\Output{\textbf{Ouput:\space}}

\usepackage{booktabs}

\usepackage{multicol}
\usepackage{tikz}
\usepackage{pgf}
\usepackage[draft,bookmarks=false]{hyperref}

\usepackage[capitalise]{cleveref}
\labelcrefformat{equation}{#2\textup{#1}#3}
% Change so that the parentheses for equations are part of the hyperlink
\creflabelformat{equation}{#2#1#3}
\crefrangelabelformat{equation}{#3#1#4 to #5#2#6}

\newcommand{\COMMENT}[1]{}

\usepackage[backend=biber,style=ieee,natbib=true]{biblatex}


==> problem_statement.tex <==
\section{Problem Statement}
In our GPS data, the majority of data is concentrated in small areas, and most road segments have no associated \gls{gps} data.
Given this discrepancy, we wish to find a model that is able to accurately assign travel times to all parts of the network, with particular emphasis on the sparsely- and unobserved areas, for the purpose of estimating route travel times in country-sized road networks.
We consider two cases: 
\begin{enumerate}
  \item The case where many road segments in a local area, e.g., a municipality, are scarcely annotated with \gls{gps} data, but some have are annotated with an abundance of data.
  \item The case where one area, e.g., a municipality, has some annotated road segments, but a distant area has no associated \gls{gps} data.
\end{enumerate}

Let $G=(V, E, A^V, A^E)$ be a directed road network where $V$ is the set of nodes, $E$ is the set of edges, and $A^V$ and $A^E$ is a set of node and edge attributes, respectively.
Let $\mathcal{T}$ be a set of \gls{gps} trips where each \emph{trip} $T_i \in \mathcal{T}$ is a sequence $T_i=\{T_{i,1}, \dots, T_{i, n}\}$. Each element $T_{i, j} \in T_i$ is an \emph{edge traversal} $(t_j, e_j, c_j)$ where $c_j$ is the cost in travel time when traversing edge $e_j$ at time $t_j$ during trip $T_i$.

Given a road network $G=(V, E, A^V, A^E)$ and a set of trips $\mathcal{T}$, we wish to find a model $f \colon E \xrightarrow{} \mathbb{R}_{>0}$ that can assign travel times to all road segments in the road network.

\christian{Define inputs, e.g., trajectory data and road network, and output (what is the model?)}


==> topmatter.tex <==
\keywords{Road Network, Machine Learning, Graph Representation Learning, Graph Convolutional Networks}

\settopmatter{printacmref=true}
% Copyright
%\setcopyright{none}
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}


% DOI
\acmDOI{10.475/123_4}

% ISBN
\acmISBN{123-4567-24-567/08/06}
\acmSubmissionID{77}

%Conference
\acmConference[SIGSPATIAL'19]{ACM SIGSPATIAL}{November 5--8 2019}
{Chicago, IL, USA}
\acmYear{2019}
\copyrightyear{2019}

%\acmPrice{15.00}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010257.10010321</concept_id>
<concept_desc>Computing methodologies~Machine learning algorithms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010405.10010481.10010485</concept_id>
<concept_desc>Applied computing~Transportation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Machine learning algorithms}
\ccsdesc[500]{Applied computing~Transportation}

